EdgeMoE: Empowering Sparse Large Language Models on Mobile Devices

Large language models (LLMs) such as GPTs and Mixtral-8x7B have revolutionized machine intelligence due to their exceptional abilities in generic ML tasks. Transiting LLMs from datacenters to edge devices brings benefits like better privacy and availability, but is challenged by their massive parameter size and thus unbearable runtime costs. To this end, we present EdgeMoE, an on-device inference engine for mixture-of-expert (MoE) LLMs -- a popular form of sparse LLM that scales its parameter size with almost constant computing complexity. EdgeMoE achieves both memory- and compute-efficiency by partitioning the model into the storage hierarchy: non-expert weights are held in device memory; while expert weights are held on external storage and fetched to memory only when activated. This design is motivated by a key observation that expert weights are bulky but infrequently used due to sparse activation. To further reduce the expert I/O swapping overhead, EdgeMoE incorporates two novel techniques: (1) expert-wise bitwidth adaptation that reduces the expert sizes with tolerable accuracy loss; (2) expert preloading that predicts the activated experts ahead of time and preloads it with the compute-I/O pipeline. On popular MoE LLMs and edge devices, EdgeMoE showcase significant memory savings and speedup over competitive baselines. The code is available at https://github.com/UbiquitousLearning/mllm.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> fig-bkgnd-infertime.tex <==
\begin{figure}[t]
	\centering
	\subfloat[Jetson TX2]{
		\includegraphics[width=0.23\textwidth]{figs/fig-inferTime-tx2.pdf}
		% \label{fig_first_case}
	}
	% \hfil
	\subfloat[Raspberry Pi 4B]{
		\includegraphics[width=0.23\textwidth]{figs/fig-inferTime-rpi4.pdf}
		% \label{fig_second_case}
	}
	%~
	%\begin{minipage}[b]{0.32\textwidth}
		%\includegraphics[width=\textwidth]{figs/TotalFrequency-ActivatedLayers_betweentokens.pdf}
		%\subcaption{Inter-token (dist=1)}
	%\end{minipage}
	\caption{
		Per-sample inference time
	}
	\label{fig:motivation-infertime}
\end{figure}

==> fig-bkgnd-metrics.tex <==
\begin{figure}[t]
	\centering					
	\includegraphics[width=0.45\textwidth]{figs/fig-bkgnd-metrics.pdf}
	%\vspace{-5pt}
	\caption{
    Accuracy(Rouge-2) loss of each single expert by quantizing them one-by-one to INT2, 
    and quantize other experts to INT4. 
    % The dataset measured is "SAMSum" 
	Model: ST-base-8. 
    Dataset: "SAMsum".
    }
	\label{fig:bkgnd-metrics}
\end{figure}

==> fig-bkgnd-weights.tex <==
\begin{figure}[t]
	\centering					
	\includegraphics[width=0.45\textwidth]{figs/fig-bkgnd-weights.pdf}
	%\vspace{-5pt}
	\caption{
		Memory usage of activated and inactive weights. 
		\yrj{remove?}
    }
	\label{fig:bkgnd-weights}
\end{figure}

==> fig-decinfertime.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{figs/fig-decInferTime-tx2.pdf}
		\subcaption{Jetson TX2}
	\end{minipage}
	~
	\begin{minipage}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{figs/fig-decInferTime-rpi4.pdf}
		\subcaption{Raspberry Pi 4B}
	\end{minipage}
	%~
	%\begin{minipage}[b]{0.32\textwidth}
		%\includegraphics[width=\textwidth]{figs/TotalFrequency-ActivatedLayers_betweentokens.pdf}
		%\subcaption{Inter-token (dist=1)}
	%\end{minipage}
	\caption{
		Per-token decoder's inference time
	}
	\label{fig:motivation-decinfertime}
\end{figure}

==> fig-design-expertpipe.tex <==
\begin{figure}[t]
	\centering					
	\includegraphics[width=0.45\textwidth]{figs/fig-design-expertpipe.pdf}
	%\vspace{-5pt}
	\caption{
		load/compute pipline of Top-3 experts.
		% X-l: X layer loading;
		% X-c: X layer computing;
	}
	\label{fig:design-expertpipe}
\end{figure}

==> fig-eval-modelsize.tex <==
\begin{figure*}[t]
	\centering					
	\includegraphics[width=0.99\textwidth]{figs/fig-eval-modelsize.pdf}
	%\vspace{-5pt}
	\caption{The model size of \sys and baselines. }
	\label{fig:eval-modelsize}
\end{figure*}

==> fig-overview.tex <==
\begin{figure}[t]
	\centering					
	\includegraphics[width=0.45\textwidth]{figs/overview}
	%\vspace{-5pt}
	\caption{An overview of \sys.}
	\label{fig:overview}
\end{figure}

==> sec-impl.tex <==
\section{Implementation and Setups}\label{sec:impl}

==> sec-measurement.tex <==
\subsection{Experimental Observations}\label{sec:measurement}
% Using 0.1\% data of full-set will enable BERT to perform on par on \texttt{AGNEWS} (0.6, 0.86), \texttt{YAHOO}(0.45, 0.66), \texttt{YELP} (0.27, 0.46), as well. While on \texttt{MNLI}, PET perform on par with CLS (0.48, 0.45). The Full-CLS are almost the same with Roberta-large.
%We emphasize necessity of big model \mwx{and its huge system cost} in Figure~\ref{fig:eval-model}.

Based on the FedFSL workflow presented above, we perform a set of early experiments on its performance.
The results highlight the two sides of a coin: a satisfactory model accuracy yet huge resource cost on clients.

\input{tab-eval-softlabel.tex}
\textit{Observation-1: FedFSL achieves satisfactory accuracy with scarce data labels; for which both pseudo labeling and prompt learning are indispensable.} 
Table~\ref{tab:eval-softlabel} shows the convergence accuracy of RoBERTa-large~\cite{liu2019roberta} on 4 popular NLP datasets\footnote{You can find a detailed description of the datasets in $\S$\ref{sec:eval-setup}.}.
With only 64 data labels (0.005\%--0.05\% of the total dataset), FedFSL achieves 85.8\%--97.0\% relatively convergence accuracy to the full-set fine-tuning that assumes all data samples are labeled.
The accuracy could be further boosted by involving more data labels.
Neither pseudo labeling nor prompt learning alone is enough to exhibit a usable accuracy.
With only one of them, the relative convergence accuracy is 40\%--74\%.
%under skewed labels distribution.
%Ours will bring less benefit under uniform distribution, while benefits still exists (from 58.1\% to 61.9\%).
Furthermore, the skewed label distribution challenges the task:
on \texttt{YELP-F}, a vanilla FedNLP method results in much higher accuracy when the labels are uniformaly distributed;
neverthelss, the challenge is mostly addressed by FedFSL that achieves satisfactory accuracy in both cases.

\input{fig-eval-model.tex}
\textit{Observation-2: FedFSL incurs huge system cost.}
Our experiments highlight the excessive system cost (Figure~\ref{fig:eval-model}), as against the commonsense that few-shot learning is usually fast and lightweight~\cite{fan2021federated, zhang2020revisiting, guha2019one, chen2019closer}.
For example, training RoBERTa-large on \texttt{AGNEWS} takes 3.3 hours to converge, 7.3 million Joules of energy, 68.4 GBs of network transmission, and 10.4 GB peak memory.
The cost is about 1.4$\times$ higher than a full-set supervised FedNLP process on the same model and dataset.
We then dive deeper into the implications behind and identify three challenges for a resource-efficient FedFSL system.
% Cost refers to energy consumption.

$\bullet$ \textbf{Orchestrating training and inference}
FedFSL has two coupled components: a federated learning runtime that continuously updates a global model; an inference runtime that keeps generating pseudo labels.
The two components must be paced harmoniously:
the inference runtime generating too few pseudo labels could slow down the training;
otherwise, generating too many pseudo labels could lead to resource waste or even excessive erroneous labels, especially when the global model is still weak.
A mechanism to orchestrate the two components must be dynamic to fit the model learning progress.

$\bullet$  \textbf{Prompt learning needs large NLP model.}
Compact NLP models have been proposed for mobile scenarios with acceptable accuracy degradation.
However, our experiments demonstrate that a large, fully-fledged foundational language model is demanded in FedFSL.
As shown in Figure~\ref{fig:eval-model}, on \texttt{MNLI} and \texttt{YELP-F}, a large RoBERTa-large model (24 transformer blocks) can reach 91\% and 88\% relative accuracy to full-set fine-tuning, while Bert-base (12 transformer blocks) can only obtain 45\% and 59\%.
The rationale is that a large language model also encodes rich knowledge for downstream tasks, from which hand-crafted prompts can better extract useful information within limited data labels.

\begin{comment}
Performance under various foundation models:
\mwx{Using 0.1\% data of full-set will enable BERT to perform on par on \texttt{AGNEWS} (0.6, 0.86), \texttt{YAHOO}(0.45, 0.66), \texttt{YELP} (0.27, 0.46), as well. While on \texttt{MNLI}, PET perform on par with CLS (0.48, 0.45). The Full-CLS are almost the same with Roberta-large.}
\end{comment}

$\bullet$ \textbf{Excessive on-device inference to obtain trustful pseudo labels.}
Pseudo labeling typically requires performing inference on all unlabeled data, from which the most confident/valuable ones can be selected for future training.
Note that the inference is not one-pass, as the model is continuously updated each round.
According to our experiments, up to 87.4\% of the total energy cost on clients is attributed to the inference.
As will be shown in $\S$\ref{sec:design-filter}, randomly filtering out a large portion of samples to speed up pseudo labeling will degrade accuracy significantly.

\begin{comment}
\cdq{Noted that} 
current pseudo labeling work selects ideal high-confidence labels from all unlabeled data.
This means inference on enormous unlabeled data is needed, which is not scalable in FL.
Related work has been widely researched in active learning~\cite{settles2009active}.
Manually annotating is costly and time-consuming.
Some samples are similar, annotating too much those similar samples would bring slight or even no benefit for subsequent training, thus wasting time and resource in vain.
What is worse, the label quality is hard to guarantee.
Naive dropping unlabeled data for pseudo labeling would harm statistical utility.
\end{comment}

==> tab-examples.tex <==

\newcommand{\OutputBoxxx}[2]{%
    \newtcolorbox{#1}{
      colback=white,
      colframe={black!65},
      title={\textbf{#2}},
      fonttitle=\bfseries,
      boxrule=0.5mm,
      arc=3mm,
      boxsep=5pt,
      left=0pt,
      right=6pt,
      top=8pt,
      bottom=8pt,
    }
}


% \section{Examples}
% Appendix one text goes here.

\OutputBoxxx{OutputBoxxxD}{Switch Transformers base-8}\label{tab:example-st}
\begin{OutputBoxxxD}
\begin{itemize}[left=0pt, label={},noitemsep,topsep=0pt]
  \item \textbf{\textcolor{blue}{Prompt:}} 
    summarize: Wellington monument on the Blackdown Hills, in Somerset, was built in 1817 but since 2005 it has been fenced off because of falling stone debris.
    The National Trust is using ground-penetrating radar on the 174ft (53m) tower to see under its stone cladding.
    Ken Evans, from the trust, said the work was "crucial".
    Built on one of the highest points of the Blackdown Hills, the landmark was put up as a tribute to the Duke of Wellington's military achievements at the Battle of Waterloo.
    But according to the trust, it has been struck by lightning twice in its history and renovating the very tall landmark every 10 to 15 years has been "expensive and unsustainable".
    Mr Evans, the trust's building surveyor, said the radar study was one of several being carried out to "understand this unique and somewhat complex monument".
    "We have been using wind and movement sensors which have already surprised us by showing that it doesn't flex in the wind quite as much as we expected," he said.
    "The ground-penetrating radar seeks to identify voids and gaps in the stonework under the surface but should also tell us more about the materials which were used to build the obelisk."
    Data from the detailed survey will also be used to build a computer model of the obelisk and help with a "more effective repair approach".
  \begin{itemize}[left=0pt,label={},noitemsep,topsep=0pt]
  \item
  \end{itemize}
    
  \item \textbf{\textcolor{orange}{original:}}
  \begin{itemize}[left=0pt,label={},noitemsep,topsep=0pt]
  \item The National Trust is studying Wellington monument on the Blackdown Hills, Somerset. The monument has been struck by lightning twice in its history. The radar study is one of several studies carried out to understand the monument.
  \end{itemize}
  
  \item \textbf{\textcolor{orange}{\sys:}}
  \begin{itemize}[left=0pt,label={},noitemsep,topsep=0pt]
  \item The National Trust is working on a project to repair Wellington monument on the Blackdown Hills, Somerset. The monument has been struck by lightning twice in its history. The project is important for the trust's building surveyor. The project will help the National Trust with the repair approach.
  \end{itemize}
\end{itemize}
\end{OutputBoxxxD}

==> tab-hitRate.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% % \usepackage{graphicx}
% \usepackage{diagbox}
\begin{table}[t]
	\centering\resizebox{\columnwidth}{!}{%
	\begin{tabular}{|@{}c|c|c|c|c@{}|}
		\hline
		\diagbox[trim=l]{num}{policy} & FIFO & LFU & LRU & Our\\		\hline
		5 & 0 & 0 & 0 & 0.2\\	\hline 
		10 & 0 & 0 & 0 & 0.2\\		\hline 
		20 & 0 & 0 & 0 & 0.2\\		\hline 
		25 & 0 & 0 & 0 & 0.2\\		\hline 
	\end{tabular} 
	}
	\label{tab:design-hitRate}
\caption{Hit ratio. "num" means the number of experts can be saved in cache memory. \mwx{TODO:translate to figure}}
\end{table}

==> tab-inferTime.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[t]
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% 		\begin{tabular}{|ll|c|c|c|}
% 			\hline
% 			\multicolumn{2}{|l|}{\textbf{MoE Architectures(GB)}} &
% 			\multicolumn{1}{l|}{\textbf{ST-base-8}} &
% 			\multicolumn{1}{l|}{\textbf{ST-base-16}} &
% 			\multicolumn{1}{l|}{\textbf{ST-base-32}} \\ \hline\hline
% 			\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{Encoder}}} &
% 			Exp. Weights 								 & 0.874      &	1.651      & 3.509     \\ \cline{2-5} 
% 			\multicolumn{1}{|l|}{} & Non-Exp. Weights    & 0.478      & 0.480      & 10.482    \\ \cline{2-5} 
% 			\multicolumn{1}{|l|}{} & Activations         & 1.758      & 2.784      & 4.520     \\ \cline{2-5} 
% 			\multicolumn{1}{|l|}{} & Total               & 3.395      & 5.038      & 9.930        \\ \hline\hline
% 			\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{Decoder}}} &
% 			Exp. Weights(Active)						 & 0.779(0.109) & 1.577(0.105) & 3.310(0.103) \\ \cline{2-5} 
% 			\multicolumn{1}{|l|}{} & Non-Exp. Weights    & 0.478         & 0.478       & 0.482         \\ \cline{2-5} 
% 			\multicolumn{1}{|l|}{} & Activations         & 1.792         & 1.861       & 1.886        \\ \cline{2-5} 
% 			\multicolumn{1}{|l|}{} & Total               & 3.684         & 4.029       & 6.276         \\ \hline
% 		\end{tabular}%
% 	}
% \caption{Memory footprint and inference latency of MoE models. ``ST'': Switch Transformers~\mwx{ref}.}
% \end{table}


\begin{table}[t]
	\centering
	\begin{minipage}[b]{0.5\textwidth}
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{l|llll}  
			\hline
			bitwidth          &FP32      &INT8     &INT4     &INT2    \\ \hline
			accuracy(rouge-2 )&0.24501   &0.24330  &0.24001  &0.20132 \\ \hline
			% load-IO(s)        &0.04899   &0.01525  &0.00765  &0.00444 \\
			% load-decompress(s)&0.00033   &0.00052  &0.00086  &0.00092 \\ \hline
			% load(s)           &0.04932   &0.01578  &0.01625  &0.01366 \\ 
			% compute(s)        &0.02779   &0.02779  &0.02779  &0.02779 \\ \hline
			token-load(s)     &0.59182   &0.18933  &0.19501  &0.16392 \\ 
			token-compute(s)  &0.16673   &0.16673  &0.16673  &0.16673 \\ \hline
			token(s)          &0.75855   &0.35606  &0.36175  &0.33065 \\ \hline
			\end{tabular} 
		}
		\subcaption{Jetson TX2}
	\end{minipage}
	
	\begin{minipage}[b]{0.5\textwidth}
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}{l|llll}  
			\hline
			bitwidth          &FP32      &INT8     &INT4     &INT2    \\ \hline
			accuracy(rouge-2 )&0.24501   &0.24330  &0.24001  &0.20132 \\ \hline
			% load-IO(s)        &0.21839   &0.05809  &0.02901  &0.01902 \\
			% load-decompress(s)&0.00675   &0.01756  &0.05579  &0.04589 \\ \hline
			% load(s)           &0.22514   &0.07565  &0.08480  &0.06491 \\ 
			% compute(s)        &0.13876   &0.13876  &0.13876  &0.13876 \\ \hline
			token-load(s)     &2.70170   &0.90781  &1.01750  &0.77893 \\ 
			token-compute(s)  &0.83256   &0.83256  &0.83256  &0.83256 \\ \hline
			token(s)          &3.53425   &1.74036  &1.85015  &1.61148 \\ \hline
			\end{tabular} 
		}
		\subcaption{Raspberry Pi 4B}
	\end{minipage}
	\caption{
		Per-token decoder's inference time. 
		"accuracy" is the rouge-2 matric. the dataset is "SAMSum". 
		The model is "switch transformer base" which is fine-tined on "SAMSum". 
		% "load-IO" and "load-decompress" means the time of IO/decompress when loading an expert's weight. 
		% "load" and "compute" means the time of load/compute for a block.  
		"token-load" and "token-compute" means the time of load/compute for a token.  
	}
	\label{tab:design-inferTime}
\end{table}

==> tab-model-memory.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{|ll|c|c|c|}
			\hline
			\multicolumn{2}{|l|}{\textbf{MoE Architectures(GB)}} &
			\multicolumn{1}{l|}{\textbf{ST-base-8}} &
			\multicolumn{1}{l|}{\textbf{ST-base-16}} &
			\multicolumn{1}{l|}{\textbf{ST-base-32}} \\ \hline\hline
			\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{Encoder}}} &
			Exp. Weights 								 & 0.874      &	1.651      & 3.509     \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Non-Exp. Weights    & 0.478      & 0.480      & 0.482    \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Activations         & 1.758      & 2.784      & 4.520     \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Total               & 3.395      & 5.038      & 9.930        \\ \hline\hline
			\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{Decoder}}} &
			Exp. Weights(Active)						 & 0.779(0.109) & 1.577(0.105) & 3.310(0.103) \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Non-Exp. Weights    & 0.478         & 0.478       & 0.482         \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Activations         & 1.792(0.150)  & 1.861       & 1.886(0.150)        \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Total               & 3.684         & 4.029       & 6.276         \\ \hline
		\end{tabular}%
	}
\caption{Memory footprint and inference latency of MoE models. ``ST'': Switch Transformers~\mwx{ref}. \mwx{the table contents need to be updated. Now it shows activation is the bottleneck, rather than the experts.}}
\label{tab:bkgnd-memory}
\end{table}

==> tab-moe-memory.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{|ll|r|r|r|}
			\hline
			\multicolumn{2}{|l|}{\textbf{MoE Architectures}} &
			\multicolumn{1}{l|}{\textbf{ST-base-16}} &
			\multicolumn{1}{l|}{\textbf{ST-base-64}} &
			\multicolumn{1}{l|}{\textbf{ST-large-128}} \\ \hline\hline
			\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Memory\\ Footprint\\ (GB)\end{tabular}}}} &
			Weights &
			100 (10\%) &
			100 (10\%) &
			100 (10\%) \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Activated Weights    & 100 (10\%) & 100 (10\%) & 100 (10\%) \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Intermediate Results & 100 (10\%) & 100 (10\%) & 100 (10\%) \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Total                & 300        & 300        & 300        \\ \hline\hline
			\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Inference\\ Time (ms)\end{tabular}}}} &
			Execution &
			10 &
			10 &
			10 \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Weights I/O          & 10         & 10         & 10         \\ \cline{2-5} 
			\multicolumn{1}{|l|}{} & Total                & 20         & 20         & 20         \\ \hline
		\end{tabular}%
	}
\caption{Memory footprint and inference latency of MoE models. ``ST'': Switch Transformers~\mwx{ref}.}
\end{table}

==> todo.tex <==
% !TeX root = main.tex 

\begin{comment}

\lwg{the key novelty of our system seems to be the dynamic expert preloading}

\lwg{compute vs computation vs computingA}

\lwg{to add the following}
\begin{myitemize}
	\item 
	Why MoE LLMs matter? Because MoE LLMs are fundamental and general: they are not arbitrary models with light modifications; they show an effective way of improving accuracy by scaling parameters but not computation. 
	
	Why MoE LLMs on edge? Why not do cloud offloading? 
	
	Hence \sys{} addresses the fundamental problem of how to execute sparse LLMs on edge devices in an memory efficient manner.  
	 
	
	\item 
	To clarify: the goal of \sys{}. 
	E.g. an accuracy goal under memory and latency constraint.
	
	\item 
	The one sentence that summarizes the key idea of \sys{}: \lwg{todo}.
	
	\item 
	Scaling parameters but not computation has been demonstrated (too strong?) to be an effective way of improving LLM performance (on edge device?). 
	Yet, the growing demands for memory of sparse LLMs pose great obstacle in their deployment on resource-constrained edge devices. 
	On one hand, large model .. cold start...;
	on the other hand, 
	
	To this end, we present \sys{}, the first system ... 
	Based on the key observation that \lwg{XXXXXX}, \sys{} systematically manages the "expert": 1) it profiles the relative importance of the expert, based on which it allocates more precisions to more important ones; 2) it instantiates a \textit{predictive loading}/execution pipeline for efficiently executing .. while attaining small memory footprints; 3) it creates an expert caching pool for ... 
	
	We show that \sys{} achieves comparable accuracy to SOTA MoE LLMs while having one to two orders of magnitude smaller memory footprints ..  
\end{myitemize}

\end{comment}
